Improving Federated Learning Personalization via Model Agnostic Meta Learning

Federated Learning (FL) refers to learning a high quality global model based on decentralized data storage, without ever copying the raw data. A natural scenario arises with data created on mobile phones by the activity of their users. Given the typical data heterogeneity in such situations, it is natural to ask how can the global model be personalized for every such device, individually. In this work, we point out that the setting of Model Agnostic Meta Learning (MAML), where one optimizes for a fast, gradient-based, few-shot adaptation to a heterogeneous distribution of tasks, has a number of similarities with the objective of personalization for FL. We present FL as a natural source of practical applications for MAML algorithms, and make the following observations. 1) The popular FL algorithm, Federated Averaging, can be interpreted as a meta learning algorithm. 2) Careful fine-tuning can yield a global model with higher accuracy, which is at the same time easier to personalize. However, solely optimizing for the global model accuracy yields a weaker personalization result. 3) A model trained using a standard datacenter optimization method is much harder to personalize, compared to one trained using Federated Averaging, supporting the first claim. These results raise new questions for FL, MAML, and broader ML research.

==> discussion_old.tex <==

% \textbf{Task and Client}
% Both MAML and FL features non-i.i.d heterogeneous local datasets~\cite{lake2015human}~\cite{caldas2018leaf}. However most FL datasets have imbalanced clients, with a few clients has much less or even no data, which makes local adaptation unstable and risky. An high quality initial model is more favorable on clients with less-than-enough data.

% \textbf{Outer Loop and Server Update} 
% Both MAML and FL aggregate gradients at each communication round, with difference on non-weighted or weighted aggregation. The server update of FL becomes more challenging, since FL gradients are corrupted intentionally to perserve differential  privacy~\cite{konevcny2016federated}.

% \textbf{Inner Loop and Client Update}
% Both MAML and FL compute gradient at each client/task. MAML algorithm computes 2nd-order gradient, 1st order approximation~\cite{finn2017model}, or simple multiple gradient descent~\cite{nichol2018first}, which can be directly applied for FL client update. Also multiple improvement on inner loop optimizers~\cite{antoniou2018train} have been proposed, which can be applied to FL client update.  

% \textbf{Gradient Steps and Local Epoch}
% MAML applies K-shot adaptation, which limits inner loop gradient steps in both meta-training and meta-testing phase. FL clients also has limited local data, but can conduct multiple epoch through the local data to optimize client performance. Comparing to MAML, FL personalization has less limitation which allows more adaptation steps. (see appendix)

% \textbf{MAML Training time and FL Convergence Speed}
% FL convergence speed is critical for deploying FL tasks, as synchronized communication requires multiple rounds to train the model. FL algorithm shows faster convergence, which can be applied to MAML algorithm for faster training.

% Canonical FL targets at training a high quality initial model, while MAML with the same algorithm structure are optimizing an initial model for fast adaptation. The similarity of MAML and FL shows that FL-training via FedAvg are actually optimizing both initial and personalization performance, which is discussed in the following sections. 

==> perf.tex <==

\begin{table}[!h]
    \centering
    \begin{tabular}{ |p{6cm}|p{3cm}|p{3cm}|}
         \hline
         EMNIST-62 Finetuning Result & Initial Acc & Personalized Acc\\
         \hline
         Adam, clr=0.02 ,Reptile(1)  &  0.7847 (0.0172)  &  0.8390 (0.0020) \\
         Adam, clr=0.005 ,Reptile(1)  &  0.7922 (0.0132)  &  0.8480 (0.0020) \\
         Momentum lr=0.01, clr=0.02, Reptile(1) & 0.7962 (0.0161) & 0.8372 (0.0027)\\
         Momentum lr=0.01, clr=0.005, Reptile(1) & 0.7830 (0.0200) & 0.8461 (0.0022)\\
         \hline
         Adam, clr=0.02 ,Reptile(2)  &  0.7894 (0.0107)  &  0.8410 (0.0020) \\
         Adam, clr=0.005 ,Reptile(2)  &  0.8042 (0.0161)  &  0.8505 (0.0020) \\
         Momentum lr=0.01, clr=0.02, Reptile(2) & 0.7990 (0.0221) & 0.8439 (0.0022)\\
         Momentum lr=0.01, clr=0.005, Reptile(2) & 0.7998 (0.0123) & 0.8542 (0.0021)\\
         \hline
         Adam, clr=0.02 ,Reptile(5)  &  0.7732 (0.0300)  &  0.8456 (0.0019) \\
         Adam, clr=0.005 ,Reptile(5)  &  0.7505 (0.0421)  &  0.8597 (0.0014) \\
         Momentum lr=0.01, clr=0.02, Reptile(5) & 0.7948 (0.0333) & 0.8491 (0.0020)\\
         Momentum lr=0.01, clr=0.005, Reptile(5) & 0.7839 (0.0363) & 0.8639 (0.0016)\\
         \hline
         Adam, clr=0.02 ,Reptile(10)  & 0.7954 (0.0238)  & 0.8501(0.0023)  \\
         Adam, clr=0.005 ,Reptile(10)  & 0.7659 (0.0401)  &  0.8670 (0.0027)  \\
         Momentum lr=0.01, clr=0.02, Reptile(10) &  0.7945(0.0337) & 0.8533 (0.0014) \\
         Momentum lr=0.01, clr=0.005, Reptile(10) & 0.7737(0.0392)  & 0.8697 (0.0013) \\
         \hline
         Adam, clr=0.02 ,Reptile(20)  &  0.7691 (0.0334) & 0.8568 (0.0014)  \\
         Adam, clr=0.005 ,Reptile(20)  & 0.7705 (0.0449)  & 0.8717 (0.0013)   \\
         Momentum lr=0.01, clr=0.02, Reptile(20) & 0.7840 (0.0199) & 0.8550 (0.0012)\\
         Momentum lr=0.01, clr=0.005, Reptile(20) & 0.7647 (0.0313)  &  0.8728 (0.0014) \\
         \hline
    \end{tabular}
    \caption{Finetuning Result of EMNIST-62}
    \label{tab:my_label}
    \vspace{-0.6cm}
\end{table}


\begin{table}[!h]
    \centering
    \begin{tabular}{ |p{6cm}|p{3cm}|p{3cm}|}
         \hline
         Shakespeare Results & Initial Acc & Personalized Acc\\
         \hline
         FedAvg $E=1$ (500 rounds)  & 0.5149  & 0.5197\\
         FedAvg $E=2$ (500 rounds)  & 0.5207  & 0.5233\\
         FedAvg $E=3$ (500 rounds)  & 0.5423  & 0.5507\\
         \hline
         Finetune with Reptile(1)  & 0.5427  & 0.5453 \\
         Finetune with Reptile(2)  & 0.5455  & 0.5484 \\
         Finetune with Reptile(5)  & 0.5489  & 0.5511 \\
         Finetune with Reptile(10)  & 0.5508  & 0.5528 \\
         \hline
    \end{tabular}
    \caption{Final Results of Shakespeare}
    \label{tab:my_label}
\end{table}

% Pers converges much faster.
\textbf{Improved persoanalized performance} Both datasets shows improved personlized performance comparing to initial performance. Table \ref{tab:my_label} shows that centralize trained model shows worse and very sensitive personlized performance comparing to FedAvg trained model, indicates FedSGD trained model has less stable personlization.
% which shows that TFF is even useful for non-FL non-iid tasks. Even you have all dataset, youn still need to train with FedAvg!

% And there should exist an optimal Epoch, but I haven't find this hyperparameter!

\textbf{Fast convergence} Both datasets trained by $FedAvg(E)$ with large enough $E$ show faster convergence in personlized performance. Personlized models reaches certain test accuracy much faster than initial model. Personalized model show much faster convergence, is useful for limited communication.

\textbf{Improved initial performance}
The personalization learning curve shows stable improvement, whereas the initial accuracy fluctuates heavily. The gradient computed via FedAvg is not mainly optimizing initial accuracy, which makes initial accuracy not stable. Finetuned by $Reptile(1)$, which is FedSGD shows best initial performance with personalized performance decreases by $0.47\%$~\cite{nichol2018first}. Different Reptile setup shows the trade-off between initial and personlized performance.


\subsection{Reducing Hyperparameter Sensitivity}
To visualize the sensitivity of personalization hyperparameters, we test multiple hyperparameter combinations on EMNIST-62. The client update learning rate range from $0.005$ to $0.1$, optimizer takes from SGD, default Adam, and Adam with $beta_1=0.0$~\cite{nichol2018first}, and client update epoch range from 1 to 10. We test the following initial models: (1) Personalized FedAvg trained model with $Reptile(1)$ trained, which has better initial accuracy, (2) Personalized FedAvg trained model with $Reptile(10)$ trained, which has better personalized accuracy, and (3) Centralized trained model with SGD. Personalized FedAvg t uses SGD with $\beta=0.02$ for client optimizer, while centralized trained model uses SGD with $\beta=0.02$ till converge. We list the best performance Table \ref{sensetable}, and plot the personalized performance of different hyperparameters in Figure \ref{senseplot}:

\begin{table}[!h]
    \centering
    \begin{tabular}{ |p{5cm}|p{1.5cm}|p{2cm}|p{3cm}|}
         \hline
         EMNIST-62 Model & Initial Acc & Pers Acc & Best Update\\
         \hline
          Personalized FedAvg Reptile(1)  & 0.8584 & 0.8784 & SGD(lr=0.02), E=5\\
          Personalized FedAvg Reptile(10) &  0.8240    & 0.8882 & SGD(lr=0.02), E=5\\
         %Centralize SGD Train Clients & 0.8459  & 0.8799 & Adam, E=10\\
         Centralize SGD Test Clients & 0.8202   & 0.8611 & Adam, E=10\\
         \hline
    \end{tabular}
    \caption{Fast adaptation sensitivity of EMNIST-62 hyperparameters}
    \label{sensetable}
    % \vspace{-1.0cm}
\end{table}


\begin{figure}[!h] 
\centering
\includegraphics[width=1.0\textwidth]{figures/client_lr_emnist_updates.png}\ \ \ 
\vspace{-0.5cm}
\caption{Hyperparameter sensitivity of personalization on EMNIST-62: centralized SGD trained model (left), and Personalized FedAvg trained model (right)}\label{senseplot}
\centering
\vspace{-0.4cm}
\end{figure}

Centralized SGD trained model are very senstivite to hyperparameters as shown in Figure \ref{senseplot} left. Other than Adam, other learning rate shows crashed performance. Still centralized SGD with Adam optimizer shows worse performance comparing Personalized FedAvg as shown in Figure \ref{senseplot} right.
Personalized FedAvg shows stable improvement, whereas the optimizer (SGD with lr=0.02) matches client training and personalization shows best performance. Adam optimizer shows worse personalized performance. Better personalized performance requires take matched client training and personalization optimizer.


\subsection{FedAvg optimize initial performance with large fluctuation}
The mean performance for initial model fluctuates a lot even after converging, which makes initial model not favorable for deployment comparing to personalized model.



\begin{table}[!h]
    \centering
    \begin{tabular}{ |p{4cm}|p{2.4cm}|p{2.7cm}|p{2.5cm}|}
         \hline
         EMNIST-62 Results bs=20 & Initial Acc & Personalized Acc & Converge Speed init/pers\\
         \hline
         FedAvg E=1, clr=0.0005  & & & \\
         FedAvg E=2, clr=0.0005  & & & \\
         FedAvg E=5, clr=0.0005 & & & \\
         FedAvg E=10, clr=0.0005 & & & \\
         FedAvg E=20, clr=0.0005 & & & \\
         \hline
         FedAvg E=1, clr=0.002  & & & \\
         FedAvg E=2, clr=0.002  & & & \\
         FedAvg E=5, clr=0.002 & & & \\
         FedAvg E=10, clr=0.002 & & & \\
         FedAvg E=20, clr=0.002 & & & \\
         \hline
          E=1, slr=0.1, clr=0.005  &  0.7903(0.0323)  & 0.8422(0.0061)& 340.6(8)/155.6(9)\\
          E=2, slr=0.1, clr=0.005  &  0.7825(0.0381)  & 0.8530(0.0046)& 286.1(9)/136.1(9)\\
          E=5, slr=0.1, clr=0.005  &  0.7666(0.0275)  & 0.8646(0.0034)& 212.5(8)/100.0(9)\\
          E=10,slr=0.1, clr=0.005 &  0.7628(0.0306)  & \textbf{0.8704(0.0017)} & 296.4(7)/100.0(9)\\
          E=20,slr=0.1. clr=0.005 &  0.7525(0.0134)  & 0.8672(0.0017) & 295.75(8)/94.4(9)\\
         \hline
          E=1, slr=1.0, clr=0.005  & 9 diverge   &  & \\
          E=2, slr=1.0, clr=0.005 & 9 diverge   &  & \\
          E=5, slr=1.0, clr=0.005  & 9 diverge  &  & \\
          E=10, slr=1.0, clr=0.005 & 0.7946(0.0398)  & 0.8484(0.0136) & 177.5(9)/50.0(9) \\
          E=20, slr=1.0, clr=0.005 & 0.7681(0.0508) & 0.8785(0.0046) & 127.5(9)/50.0(8) \\
         \hline
          E=1, slr=0.1, clr=0.02  &  0.7918(0.0239)  & 0.8491(0.0019) & 280.6(9)/127.8(9)\\
          E=2, slr=0.1, clr=0.02  &  0.7839(0.0471)  & 0.8525(0.0020) & 275.0(9)/122.2(9)\\
          E=5, slr=0.1, clr=0.02  &  0.7432(0.0212)  & \textbf{0.8546(0.0021)} & 346.42(7)/108.3(9)\\
          E=10, slr=0.1, clr=0.02 &  0.7679(0.0255)  & 0.8509(0.0024) & 433.3(3)/105.0(8)\\
          E=20, slr=0.1, clr=0.02 &  0.7503(0.0115)  & 0.8437(0.0022) & Never/132.5(9)\\
         \hline
          E=1, slr=1.0, clr=0.02  & 9 Diverged  &  & \\
          E=2, slr=1.0, clr=0.02  & 1 Diverged  &  & \\
          E=5, slr=1.0, clr=0.02  &  0.8028 (0.0512)  & 0.8712 (0.0049)  & 111.1(9)/50.0(9) \\
          E=10, slr=1.0, clr=0.02 & 0.7879(0.0316)  & \textbf{0.8820 (0.0023)} & 138.63(9)/50.0(9)\\
          E=20, slr=1.0, clr=0.02 &  0.7430(0.0309) & 0.8782 (0.0021) & 152.5(8)/50.0(9) \\
         \hline
         
         
         FedAvg E=1, clr=0.05  &  0.8045(0.0210)  & 0.8370(0.0025) & 277.7(8)/165.0(9)\\
         FedAvg E=2, clr=0.05  &  0.7851(0.0266)  & 0.8401(0.0018) & 313.9(9)/152.8(9)\\
         FedAvg E=5, clr=0.05  &  0.7752(0.0220)  & 0.8410(0.0025) & 437.5(6)/155.6(9)\\
         FedAvg E=10, clr=0.05 &  0.7585(0.0143)  & 0.8388(0.0023) & Never/163.9(9) \\
         FedAvg E=20, clr=0.05 &  0.7457(0.0120)  & 0.8282(0.0022) & Never/222.2(6)\\
         \hline
    \end{tabular}
    \caption{Personalized Performance is more stable than initial model with 9 runs for each experiment. Also the convergence speed is shown with average round of communications to reach accuracy 0.8, with number of reached runs marked in (). }
    \label{seenclient}
    \vspace{-0.6cm}
\end{table}

Train acc equals personalized acc, for validating dataset?


For fixed client the initial performance is jumping a lot alsoeven after convergence. visualize for both finetune Reptile and FedAvg.


\subsection{Client Learning Rate}
Client learning rate is critical hyperparameter for FL personalization. 

We find $lr=0.005$ is good.

In terms of fast convergence


\subsection{Batch size effects}
Running the same experiment on batch size 20 and 100 shows different performance.



\subsection{Smaller Model effects}
Smaller model with small bottlenectk units, show degraded performance, with much smaller personalization improvement. Which means at least reduce bottleneck unit makes it worse...



\subsection{Unstable Small Step Finetuning: Use Adam server optimizer}
More local epoch shows to be more stable for FL learning than Reptile, which is 

Finetuning result (client learning rate 0.02, )




\begin{table}[!h]
    \centering
    \begin{tabular}{ |p{7cm}|p{2.5cm}|p{2.5cm}|}
         \hline
         EMNIST-62 Model & Initial Acc & Pers Acc\\
         \hline
         Initial Model without finetuning & 0.7441   & 0.8842 \\
         \hline
         Reptile(1) SGD(0.1) 100 rounds &  0.8292(0.0188)   & 0.8764 (0.0026)  \\
         Reptile(1) Momentum(0.01, 0.9) 100 rounds &  0.8285 (0.0186) &  0.8760 (0.0022) \\
         Reptile(1) Adam 100 rounds &  0.8240 (0.0085)   & 0.8760 (0.0018) \\
         
         \hline
         Reptile(1) SGD(0.1) 200 rounds & 0.8260 (0.0161) & 0.8758 (0.002) \\
         Reptile(1) Momentum(0.01, 0.9) 200 rounds & 0.8279 (0.0119) & 0.8745 (0.0014)\\
         Reptile(1) Adam 200 rounds &  \textbf{0.8320 (0.0133)}   &  0.8764 (0.0017)  \\
         
         \hline
         Reptile(5) SGD(0.1) 100 rounds &  0.8082 (0.0381)& 0.8817 (0.0016) \\
         Reptile(5) Momentum(0.01, 0.9) 100 rounds & 0.8128 (0.0382) & 0.8825 (0.0012) \\
         Reptile(5) Adam 100 rounds & 0.8212 (0.0175)   &  0.8801 (0.0022)\\
         
         \hline
         Reptile(5) SGD(0.1) 200 rounds & 0.8148 (0.0280)  & 0.8829 (0.0012) \\
         Reptile(5) Momentum(0.01, 0.9) 200 rounds & 0.8005 (0.0329)  &  0.8828 (0.0015) \\
         Reptile(5) Adam 200 rounds &  \textbf{0.8265 (0.0160)} & 0.8807 (0.0020)\\
         

         \hline
         Reptile(10) SGD(0.1) 100 rounds & 0.8057(0.0257) & 0.8849 (0.0011) \\
         Reptile(10) Momentum(0.01, 0.9) 100 rounds & 0.7943 (0.0282) & 0.8840 (0.0009) \\
         Reptile(10) Adam 100 rounds & 0.8049 (0.0275) &     0.8843 (0.0026)\\
         
         \hline
         Reptile(10) SGD(0.1) 200 rounds & 0.8074 (0.0294) & 0.8855 (0.0012)\\
         Reptile(10) Momentum(0.01, 0.9) 200 rounds &  0.8140 (0.0246) & 0.8864 (0.0009)  \\
         Reptile(10) Adam 200 rounds &  \textbf{0.8116 (0.0148)} & 0.8858 (0.0014)\\
         \hline
         Reptile(1) Adam 200 rounds &  \textbf{0.8320 (0.0133)}   &  0.8764 (0.0017)  \\
         Reptile(5) Adam 200 rounds &  \textbf{0.8265 (0.0160)} & 0.8807 (0.0020)\\
         Reptile(10) Adam 200 rounds &  \textbf{0.8116 (0.0148)} & 0.8858 (0.0014)\\
         \hline
    \end{tabular}
    \caption{Fine-tuning Result of EMNIST-62 hyperparameters}
    \label{sensetable}
    % \vspace{-1.0cm}
\end{table}


\subsection{Personlized Client Performance (Fairness)}
Testing on the client not seen during training, we visualize the client test performance as shown in Figure \ref{clientscatter}. There is no clear sign of unfairness, as the client with more dataset are not necessarily show worse performance.

\begin{figure}[!h] 
\centering
\includegraphics[width=1.0\textwidth]{figures/scatter.png}\ \ \ 
\caption{Performance for test clients for EMNIST-62 and Shakespeare}\label{nonawgn}
\centering
\end{figure}\label{clientscatter}

\subsubsection{Negative Personalization Effects}
We term reduced performance after personalization as negative personalization. The goal is to avoid negative personalization as much as possible.

For EMNIST-62, Reptile (1) finetuned model has , while Reptile(10) finetuned model has negative personalization. 


Epoch with accuracy and positive personalization propotion.











